Magnifying Lens Abstraction for Stochastic Games with Discounted and Long-run Average Objectives

Turn-based stochastic games and its important subclass Markov decision processes (MDPs) provide models for systems with both probabilistic and nondeterministic behaviors. We consider turn-based stochastic games with two classical quantitative objectives: discounted-sum and long-run average objectives. The game models and the quantitative objectives are widely used in probabilistic verification, planning, optimal inventory control, network protocol and performance analysis. Games and MDPs that model realistic systems often have very large state spaces, and probabilistic abstraction techniques are necessary to handle the state-space explosion. The commonly used full-abstraction techniques do not yield space-savings for systems that have many states with similar value, but does not necessarily have similar transition structure. A semi-abstraction technique, namely Magnifying-lens abstractions (MLA), that clusters states based on value only, disregarding differences in their transition relation was proposed for qualitative objectives (reachability and safety objectives). In this paper we extend the MLA technique to solve stochastic games with discounted-sum and long-run average objectives. We present the MLA technique based abstraction-refinement algorithm for stochastic games and MDPs with discounted-sum objectives. For long-run average objectives, our solution works for all MDPs and a sub-class of stochastic games where every state has the same value.

==> mla.tex <==
\subsection{Magnifying-Lens Abstraction (MLA)}
\label{sec-mla}
\noindent
{\em Magnifying-lens abstractions\/} (MLA) \cite{deAlR07} is a technique for the
analysis of reachability and safety properties of MDPs.
MLA can cluster states based on value only, disregarding differences in their transition relation.
This feature can lead to compact abstractions for systems where full abstraction provides no
benefit. 
In our experience, MLA is particularly well-suited to problems where
there is a notion of {\em locality\/} in the state space, so that it
makes sense to cluster states based on variable values --- even though
their transition relations may not be similar. 
Many inventory, planning and control problems are of this type. 
%MLA is not, however, as well-suited to problems where clustering states
%based on variable values is less effective. 



Let $v^*$ be the valuation over $S$ that is to be computed: 
$v^*$ is one of 
$V^{\min}_{\Box T}$, 
$V^{\max}_{\Box T}$, 
$V^{\min}_{\Diamond T}$, 
$V^{\max}_{\Diamond T}$.
Given a desired accuracy $\veabs {>} 0$, MLA
computes upper and lower bounds for $v^*$, spaced less than $\veabs$ apart.
MLA starts from an initial partition (set of regions) $R$ of $S$.
The initial partition $R$ is obtained either from the user or from the property. 
 MLA computes the lower and upper bounds as valuations 
$u^-$ and $u^+$ over $R$. 
The partition is refined, until the difference between $u^-$ and
$u^+$, for all regions, is below a specified threshold. 
To compute $u^-$ and $u^+$, MLA iteratively considers each region $r \in R$ in
turn, and performs a {\em magnified iteration:\/} it improves the
bounds $u^-(r)$ and $u^+(r)$ by performing value iteration on the
concrete states in $r$.

The MLA algorithm is shown in Algorithm~\ref{algo-mla}.
The algorithm has parameters $T$, $\opnext$, $\opact$, which have the
same meaning as ValIter in Algorithm~\ref{valueiteration}. 
The algorithm also has parameters $\vefloat {>} 0$ and $\veabs {>} 0$.
Parameter $\veabs$ indicates the maximum difference between the lower
and upper bounds returned by MLA. 
Parameter $\vefloat$, as in~ValIter, specifies the degree of precision
to which the local, magnified value iteration should converge. 
MLA should be called with $\veabs$ greater than $\vefloat$ by at least
one order of magnitude: otherwise, errors in the magnified
iteration can cause errors in the estimation of the bounds.
%
Statement 2 initializes the valuations $u^-$ and $u^+$ according to
the property to be computed: reachability properties are computed as
least fixpoints, while safety properties are computed as greatest
fixpoints \cite{dAM04}.  
%
A region $r_2$ is called successor to a region $r_1$ if at least one concrete state
in $r_1$ has non-zero probability to reach concrete state(s) in $r_2$.
A useful time optimization, not shown in Algorithm~\ref{algo-mla}, 
consists in executing the loop at lines 6--9 only for regions $r$
where at least one of the successor regions has changed value by more
than $\vefloat$. 

\begin{algorithm}[t]
\caption{MLA$(T,\opnext,\opact,\vefloat,\veabs)$ Magnifying-Lens Abstraction}
\label{algo-mla}
\begin{tabbing}
1.     \quad \= $R {:=}$ some initial partition. \\
2.  \> {\bf if} $\opnext {=} \max$ 
          {\bf then} $u^- {:=} \mathbf{0}$; $u^+ {:=} \mathbf{0}$
          {\bf else} $u^- {:=} \mathbf{1}$; $u^+ {:=} \mathbf{1}$ \\
3.  \> {\bf loop} \\
4.  \> {\bf if} $\opnext {=} \max$ {\bf then} $u^+$ {:=} $u^-$ {\bf else}  $u^-$ {:=} $u^+$\\
5.  \> \quad {\bf repeat} \\
6.  \> \quad \quad $\hat{u}^+ {:=} u^+$; $\hat{u}^- {:=} u^-$; \\
7.  \> \quad \quad {\bf for} $r \in R$ {\bf do}\\
8.  \> \quad \quad \quad $u^+(r) {:=}$ MI$(r,R,T,\hat{u}^+,\hat{u}^-,\hat{u}^+,\max,\opnext,\opact,\vefloat)$\\
9.  \> \quad \quad \quad $u^-(r) {:=}$ MI$(r,R,T,\hat{u}^-,\hat{u}^-,\hat{u}^+,\min,\opnext,\opact,\vefloat)$\\
10.  \> \quad \qquad {\bf end for} \\
11. \> \quad {\bf until} $\max(||u^+ - \hat{u}^+||,||u^- - \hat{u}^-||) \leq \vefloat$ \\
12. \> \quad {\bf if} $||u^+ - u^-|| \geq \veabs$ \\
13. \> \quad \quad {\bf then} $R, u^-, u^+ {:=}$ SplitRegions$(R,u^-,u^+,\veabs)$ \\
14. \> \quad \quad {\bf else} {\bf return} $R, u^-, u^+$ \\
15. \> \quad {\bf end if} \\
16. \> {\bf end loop}
\end{tabbing}
\vspace*{-2ex}
\end{algorithm}
%
\begin{algorithm}[t]
\caption{MI$(r,R,T,u,u^-,u^+,h,\opnext,\opact,\vefloat)$} 
  \label{algo-local}
\begin{tabbing}
$v$: a valuation over $r$ \\
1.  \= {\bf if} $\opnext {=} \max$ \\
2.  \> \quad {\bf then} {\bf for} $s \in r$ {\bf do} $v(s) {=} u^-(r)$ \\
3.  \> \quad {\bf else} {\bf for} $s \in r$ {\bf do} $v(s) {=} u^+(r)$ \\
4.  \> {\bf repeat} \\
5.  \> \quad $\hat{v} {:=} v$ \\
6.  \> \quad {\bf for all} $s \in r$ {\bf do} \\
6a.\> \quad $\displaystyle
       t {=} \opact_{a \in \Gamma(s)} \biggl\{ 
        \mbox{$\sum\limits_{s'\in r}$} p(s,a,s')\cdot\hat{v}(s')$ \\
    \> \quad $\displaystyle \qquad \qquad \qquad + \mbox{$\sum\limits_{s'\in S \setm r}$} p(s,a,s') \cdot u([s]_R) 
      \biggr\}$ \\[0.5ex]
6b.\> \quad $v(s) {:=}  \opnext \Biggl([T](s),t \Biggr)$\\
7.  \> {\bf until} $||v - \hat{v}|| \le \vefloat$ \\[0.5ex]
8.  \> {\bf return} $h \set{v(s) \mid s \in r}$
\end{tabbing}
\vspace*{-2ex}
\end{algorithm}

\paragraph{Magnified iteration.} 

The algorithm performing the magnified iteration is given in 
Algorithm~\ref{algo-local}. 
This is very similar to ValIter in Algorithm~\ref{valueiteration},
except for three points. 

First, the valuation $v$ (which here is local to $r$) is initialized
not to $[T]$, but rather, to $u^-(r)$ if $\opnext {=} \max$, and to
$u^+(r)$ if $\opnext {=} \min$. 
Indeed, if $\opnext {=} \max$, value iteration converges from below, and
$u^-(r)$ is a better starting point than $[T]$, since $[T](s) \leq
u^-(r) \leq v^*(s)$ at all $s \in r$. 
The case for $\opnext {=} \min$ is symmetric. 

Second, for $s \in S \setm r$, the algorithm uses, in place of the
value $v(s)$ which is not available, the value $u^-(r')$ or $u^+(r')$,
as appropriate, where $r'$ is such that $s \in r'$.
In other words, the algorithm replaces values at concrete states
outside $r$ with the ``abstract'' values of the regions to which the
states belong. 
To this end, we need to be able to efficiently find the ``abstract''
counterpart $[s]_R$ of a state $s \in S$.
We use the following scheme, similar to schemes used in AMR (adaptive mesh refinement)
\cite{BergerOliger84}. 
The state-space $S$ of the MDP consists of value
assignments to a set of variables $X = \set{x_1, x_2, \ldots, x_l}$.
In \cite{deAlR07} we represented a partition $R$ of $S$, together with the valuations $u^+$,
$u^-$, via a binary decision tree.
The leaves of the tree correspond to regions, and they are labeled
with $u^-$, $u^+$ values. 
Given $s$, finding $[s]_R$ in such a tree requires time logarithmic in
$|S|$.  

Third, once the concrete valuation $v$ is computed at all $s \in r$,
Algorithm~\ref{algo-local} returns the minimum (if $h {=} \min$) or the
maximum (if $h {=} \max$) of $v(s)$ at all $s \in r$, thus providing a
new estimates for $u^-(r)$, $u^+(r)$, respectively. 


\paragraph{Adaptive abstraction refinement.}

We denote the {\em imprecision\/} of a region $r$ by 
$\Delta(r) = u^+(r) - u^-(r)$. 
MLA adaptively refines a partition $R$ by splitting all regions $r$
having $\Delta(r) > \veabs$.
This is perhaps the simplest possible refinement scheme. 
We have experimented with alternative refinement schemes, but none
were consistently better \cite{deAlR07}. 

As previously explained, the partition $R$ is represented by a decision tree,
whose leaves correspond to the regions.
In the refinement phase, we split a leaf according to the value of a
new variable (not present in that leaf), following the variable ordering
given by the user.


 
A call to SplitRegions$(R,u^+,u^-,\veabs)$ returns a triple 
$\tilde{R}, \tilde{u}^-, \tilde{u}^+$, consisting of the new
partition with its upper and lower bounds for the valuation. 


\paragraph{Correctness.} The following theorem summarizes the correctness of the MLA algorithm.
\begin{theorem}\cite{deAlR07}
For any MDP $M = \langle S, s_{init}, A, \Gamma, p \rangle$, set of states $T \subs S$,
and error bound $\veabs {>} 0$, the following assertions hold. 
%
\begin{enumerate}
\item {\em Termination.}  For all $\vefloat {>} 0$ and $\opnext, \opact \in \set{\min,\max}$, 
the call MLA$(T,\opnext,\opact,\vefloat,\veabs)$ terminates. 

\item {\em (Partial) correctness.}  
  Let $\opact \in \set{\max,\min}$, $\veabs {>} 0$ and 
  $\bigtriangleup \in \set{\Box,\Diamond}$. If 
  $\opnext {=} \min$ when $\bigtriangleup {=} \Box$, and $\opnext {=} \max$ when
  $\bigtriangleup {=} \Diamond$, then for all $\delta {>} 0$, there exists $\vefloat {>} 0$ such that:
%
\begin{align*}
  & \forall r \in R: & & u^+(r) {-} u^-(r) \leq \veabs \\
  & \forall s \in S: & & u^-([s]_R) {-} \delta \leq V^\opact_{\bigtriangleup T}(s) \leq u^+([s]_R) {+} \delta
\end{align*}
%
where $(R,u^-,u^+) = \mbox{MLA}(T,\opnext,\opact,\vefloat,\veabs)$.

\end{enumerate}
\end{theorem}

\noindent
We note that the theorem establishes the correctness of lower and
upper bounds only within a constant $\delta {>} 0$, which depends on
$\vefloat$. 
This limitation is inherited from the value-iteration scheme used over
the magnified regions.
If linear programming \cite{Derman,Bertsekas95} were used instead,
then MLA would provide true lower and upper bounds. 
However, in practice value iteration is preferred over linear
programming, due to its simplicity and greater efficiency, and the
concerns about $\delta$ are solved - in practice, albeit not in
theory - by choosing a sufficiently small $\vefloat$.
%\gethinnote{more important linear programming cannot be applied to large systems? perhaps not for mla}
%\mynote{i do not think we need to elaborate this part}

